Exploiting the Distortion-Semantic Interaction in Fisheye Data

In this work, we present a methodology to shape a fisheye-specific representation space that reflects the interaction between distortion and semantic context present in this data modality. Fisheye data has the wider field of view advantage over other types of cameras, but this comes at the expense of high radial distortion. As a result, objects further from the center exhibit deformations that make it difficult for a model to identify their semantic context. While previous work has attempted architectural and training augmentation changes to alleviate this effect, no work has attempted to guide the model towards learning a representation space that reflects this interaction between distortion and semantic context inherent to fisheye data. We introduce an approach to exploit this relationship by first extracting distortion class labels based on an object's distance from the center of the image. We then shape a backbone's representation space with a weighted contrastive loss that constrains objects of the same semantic class and distortion class to be close to each other within a lower dimensional embedding space. This backbone trained with both semantic and distortion information is then fine-tuned within an object detection setting to empirically evaluate the quality of the learnt representation. We show this method leads to performance improvements by as much as 1.1% mean average precision over standard object detection strategies and .6% improvement over other state of the art representation learning approaches.

==> Sections/archive.tex <==

\twocolumn[{%
\vspace{20mm}
%\renewcommand\twocolumn[1][]{#1}%
{ \large
\begin{itemize}[leftmargin=2.5cm, align=parleft, labelsep=2cm, itemsep=4ex,]

\item[\textbf{Citation}]{K. Kokilepersaud, M. Prabhushankar, Y. Yarici, G. AlRegib, and A. Mostafa, "Exploiting the Distortion-Semantic Interaction in Fisheye Data" in \textit{Open Journal of Signals Processing}, 2023.}

\item[\textbf{Review}]{Date of Publication: May 1st 2023}

\item[\textbf{Codes}]{\url{https://github.com/olivesgatech/Image-2022-Volumetric-Contrastive.git}}


\item[\textbf{Bib}]  {@inproceedings\{kokilepersaud2022exploiting,\\
    title=\{Exploiting the Distortion-Semantic Interaction in Fisheye Data\},\\
    author=\{K. Kokilepersaud, M. Prabhushankar, Y. Yarici, G. AlRegib, and A. Mostafa\},\\
    booktitle=\{Open Journal of Signals Processing\},\\
    year=\{2023\}\}}

%\item[\textbf{Copyright}]{\textcopyright 2022 IEEE. Personal use of this material is permitted. Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting/republishing this material for advertising or promotional purposes,
%creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component
%of this work in other works.}

\item[\textbf{Contact}]{
\{kpk6, mohit.p, alregib\}@gatech.edu\\
\url{https://ghassanalregib.info/}\\}
\end{itemize}
}}]
% \thispagestyle{empty}
\newpage
